Audio2Face-3D: Audio-driven Realistic Facial Animation For Digital Avatars

Audio-driven facial animation presents an effective solution for animating digital avatars. In this paper, we detail the technical aspects of NVIDIA Audio2Face-3D, including data acquisition, network architecture, retargeting methodology, evaluation metrics, and use cases. Audio2Face-3D system enables real-time interaction between human users and interactive avatars, facilitating facial animation authoring for game characters. To assist digital avatar creators and game developers in generating realistic facial animations, we have open-sourced Audio2Face-3D networks, SDK, training framework, and example dataset.

==> figures/10_future/fig_A2FR_network.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/10_future/a2r_v4.pdf}
    \caption{A2F-Rig model architecture.}
    \label{fig:A2FR_network}
\end{figure}

==> figures/10_future/fig_result_emo_trans.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/10_future/result_emo_trans.png}
    \caption{The results of emotion transition.}
    \label{fig:results_emo_trans}
\end{figure}


==> figures/10_future/fig_results_tex_cond_backup.tex <==
%\begin{figure}[H]
%    \centering
%    \includegraphics[width=0.8\textwidth]{images/10_future/result_text_cond.png}
%    \caption{The results of text-driven emotion and facial movement control.}
%    \label{fig:results_text_cond}
%\end{figure}


%#tOUrism, conTribution,  Four   tWenty  SEven      bhAt  thirtEEn    Billion,  tEn
%#   8        117          276   328      343       433       491        551       677

% tabulars
\setlength{\rowlabelwidth}{0.12\textwidth}

\begin{figure}[H]
\definecolor{PromptGray}{gray}{0.6}

\setlength{\tabcolsep}{0pt} % Remove column separation
\renewcommand{\arraystretch}{0.5} % Remove row separation

\newcommand{\xdownarrow}[1]{\mathrel{\rotatebox{-90}{$\xrightarrow{#1}$}}}
\newcommand{\promptText}[1]{\textcolor{PromptGray}{\small \emph{#1}}}

% EMOTION CONTROL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{flushleft}
%\emph{(a) Emotion Control}
(a) Emotion Control
\end{flushleft}
\centering
\begin{tabular}{m{4cm} c c c c c c }
%& \emph{\nvGreen{f}oot} & \emph{\nvGreen{w}ear} & \emph{wea\nvGreen{r}} & \emph{cow\nvGreen{b}oy} & \emph{\nvGreen{ch}aps}  & \emph{\nvGreen{m}oving} \\[0.3em]

& \emph{t\nvGreen{OU}rism} & \emph{con\nvGreen{T}ribution} & \emph{\nvGreen{F}our} & \emph{t\nvGreen{WE}nty} & \emph{\nvGreen{SE}ven}  & \emph{bh\nvGreen{A}t} \\[0.3em]

\promptText{``a person looks joyful''} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_neutral_0064.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_amazement_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_joy_0073.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_disgust_0102.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_anger_0107.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_fear_0169.png}} \\ [-0.5em]
\promptText{``a person is amazed''} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_neutral_0064.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_amazement_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_joy_0073.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_disgust_0102.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_anger_0107.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_fear_0169.png}} \\
\promptText{``a person is disgusted''} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_neutral_0064.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_amazement_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_joy_0073.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_disgust_0102.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_anger_0107.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_fear_0169.png}} \\ [-0.5em]
\promptText{``a person is lonely''}  &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_neutral_0064.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_amazement_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_joy_0073.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_disgust_0102.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_anger_0107.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_fear_0169.png}} \\
\end{tabular}\\[0.3em]

\textcolor{gray!60}{\rule{\textwidth}{1pt}}\\[0.3em]

% FACIAL MOVEMENT CONTROL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{flushleft}
%\emph{(b) Facial Movement Control}
(b) Facial Movement Control
\end{flushleft}
\begin{tabular}{m{4cm} c c c c c c }
\parbox{3.75cm}{\promptText{``a person appears neutral and speaks with smiling mouth''}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_neutral_0064.png}}   &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_amazement_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_joy_0073.png}}       &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_disgust_0102.png}}   &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_anger_0107.png}}     &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/mark_fear_0169.png}}      \\ [-0.5em]
\parbox{3.75cm}{\centering\promptText{``a person appears neutral and speaks with furrowed eyebrows''}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_neutral_0064.png}}   &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_amazement_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_joy_0073.png}}       &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_disgust_0102.png}}   &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_anger_0107.png}}     &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/claire_fear_0169.png}}     \\
\end{tabular}\\[0.3em]

\textcolor{gray!60}{\rule{\textwidth}{1pt}}\\[0.3em]

% INTENSITY CONTROL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{flushleft}
%\emph{(c) Intensity Control}
(c) Intensity Control
\end{flushleft}
\begin{tabular}{m{4cm} c c c c c c }
%\parbox{4cm}{\centering\textcolor{PromptGray}{\shortstack[c]{``a person looks angry''\\$\xdownarrow{}$\\``a person looks extremely angry''}}}&
%\textcolor{PromptGray}{``a person looks angry'' $\xrightarrow{}$ ``a person looks extremely angry''} &
\parbox{4cm}{ \centering \promptText{%
   ``a person looks angry''\\
   \vspace{-1em} $\xdownarrow{}$\\
  ``a person looks extremely angry''
}}&
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0064.png}}  &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0073.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0102.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0107.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0112.png}} \\
& \emph{\footnotesize \strut Anger } &
\multicolumn{4}{c}{%
\tikz[baseline]{
  \draw[->, thick, color=nvidiagreen, line width=2pt, >=stealth]
    (0,0) -- (3.95*\rowlabelwidth,0);
}
} &
\emph{\footnotesize \strut Extreme anger} \\
\end{tabular}

\vspace{0.3em}

\textcolor{gray!60}{\rule{\textwidth}{1pt}}\\[0.3em]

% EMOTION TRANSITION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{flushleft}
%\emph{(d) Emotion Transitions}
(d) Emotion Transitions
\end{flushleft}
\begin{tabular}{m{4cm} c c c c c c }
\parbox{4cm}{ \centering \promptText{%
\shortstack[c]{``a person looks joyful''\\$\xdownarrow{}$\\``a person looks angry''}}}&
%\textcolor{PromptGray}{``a person looks joyful'' $\xrightarrow{}$ ``a person looks angry''} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0064.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0070.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0073.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0102.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0107.png}} &
\CenterImage{\includegraphics[width=\rowlabelwidth]{images/7_results/fig_emotions/james_joyToAnger_0112.png}} \\
& \emph{\footnotesize \strut Joy } &
\multicolumn{4}{c}{%
\tikz[baseline]{
  \draw[->, thick, color=nvidiagreen, line width=2pt, >=stealth]
    (0,0) -- (3.95*\rowlabelwidth,0);
}
} &
\emph{\footnotesize \strut Anger} \\
\end{tabular}

\caption{ \red{W.I.P. layout done - need to update images } The results of text-driven emotion and facial movement control. The leftmost text indicates the prompt used to generate the facial animation.}
\label{fig:results_text_cond}
\end{figure}

==> figures/7_results/fig_results_bs_solve_error.tex <==
\setlength{\rowlabelwidth}{0.13\textwidth}

\begin{figure}[H]
\centering
\setlength{\tabcolsep}{0.0pt}
\renewcommand{\arraystretch}{0}
\begin{tabular}{c c c c c c c c}
 & \emph{t\nvGreen{e}nure} & \emph{S\nvGreen{u}zie} & \emph{\nvGreen{a}ll} & \emph{l\nvGreen{ei}sure} & \emph{\nvGreen{f}or} & \emph{y\nvGreen{a}tching} & \\[0.3em]
\rotatebox{90}{\makebox[0pt][l]{\emph{\small Error}}} \hspace{0.1em} &
\includegraphics[width=\rowlabelwidth]{images/7_results/fig_bs_solve/james_comp_20.png} &
\includegraphics[width=\rowlabelwidth]{images/7_results/fig_bs_solve/james_comp_40.png} &
\includegraphics[width=\rowlabelwidth]{images/7_results/fig_bs_solve/james_comp_60.png} &
\includegraphics[width=\rowlabelwidth]{images/7_results/fig_bs_solve/james_comp_77.png} &
\includegraphics[width=\rowlabelwidth]{images/7_results/fig_bs_solve/james_comp_84.png} &
\includegraphics[width=\rowlabelwidth]{images/7_results/fig_bs_solve/james_comp_94.png} &
\begin{tikzpicture}
\begin{axis}[
    hide axis,
    scale only axis,
    height=0.13\textwidth,    
    colorbar,
    colormap/jet,
    point meta min=0,
    point meta max=8,
    colorbar style={
        width=0.01\textwidth,
        ytick={0,4,8},
        yticklabels={0 mm, 4 mm, 8 mm},
        tick label style={font=\tiny}
    }
]
\addplot [draw=none] coordinates {(0,0)};
\end{axis}
\end{tikzpicture}
\end{tabular}
\caption{Error between blendshape solve and inference}
\label{fig:results_bs_error}
\end{figure}

==> tables/3_data/summary_training_data.tex <==
\begin{table}[H]
    \setlength{\tabcolsep}{4.7pt}
    \small
    \captionsetup{justification=centering}
    \caption{Summary of the training parameters for each facial component}
    \centering
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{ r  c  c } 
     \toprule
     Facial component & Training parameters & Dimension  \\
     \midrule
     skin & PCA parameters & 140 \\ 
    
     tongue & PCA parameters & 10 \\
     
     jaw & delta of 5 points & 15 \\
    
     eyeballs & yaw and pitch (left, right) & 4 \\ 
     \bottomrule
    \end{tabular}
    
    \label{tab:summar_training_data}
\end{table}
